Time-Varying Semidefinite Programs

We study time-varying semidefinite programs (TV-SDPs), which are semidefinite programs whose data (and solutions) are functions of time. Our focus is on the setting where the data varies polynomially with time. We show that under a strict feasibility assumption, restricting the solutions to also be polynomial functions of time does not change the optimal value of the TV-SDP. Moreover, by using a Positivstellensatz on univariate polynomial matrices, we show that the best polynomial solution of a given degree to a TV-SDP can be found by solving a semidefinite program of tractable size. We also provide a sequence of dual problems which can be cast as SDPs and that give upper bounds on the optimal value of a TV-SDP (in maximization form). We prove that under a boundedness assumption, this sequence of upper bounds converges to the optimal value of the TV-SDP. Under the same assumption, we also show that the optimal value of the TV-SDP is attained. We demonstrate the efficacy of our algorithms on a maximum-flow problem with time-varying edge capacities, a wireless coverage problem with time-varying coverage requirements, and on bi-objective semidefinite optimization where the goal is to approximate the Pareto curve in one shot.

==> definitions/expression_F_star.tex <==
$$F^*P(t) \coloneqq \begin{pmatrix}\langle A_0(t), P(t) \rangle\\ \langle A_1(t), P(t) \rangle + \int_t^1 \langle D_1(s, t), P(s) \rangle \;{\rm d}s \\\vdots\\ \langle A_n(t), P(t) \rangle + \int_t^1 \langle D_n(s, t), P(s) \rangle \;{\rm d}s\end{pmatrix}.$$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../TV_SDP_v1"
%%% End:


==> old_proofs.tex <==



It is already known that a sequence of bounded measures on a compact set has subsequence that converges weakly as the following theorem formalizes.
\begin{thm}
  \label{thm:bounded.measure.compact}
  If $\{\mu_n\}$ is a sequence of measures in $\measureset$ and $c$ a positive constant such that
  \begin{equation}
    \label{eq:bounded.measure}
    |\mu_n(f)| \le c \sup_{t \in [0, 1]} \|f(t)\|_\infty \quad \forall f \in \LintRn,
  \end{equation}
  then there exists $\mu \in \measureset$ and subsequence $\{\mu_{i_n}\}$ of $\{\mu_n\}$ such that
  $$\mu_{i_n} \weakcvg \mu \text{ as } n \rightarrow \infty,$$
  and
  $$|\mu(f)| \le c \sup_{t \in [0, 1]} \|f(t)\|_\infty \quad \forall f \in \LintRn.$$
\end{thm}

The following theorem shows that when these measures have densities (i.e. are absolutely continuous with respect to the Lebesgue measure), then the limit is also absolutely continuous.

\begin{thm}
(See \cite{WeakConvergenceUniformBound})
Suppose $(d\mu_k = f_k dt)_k$ is a sequence of measures of $\measureset$ and \(M\) a positive constant such that $$\|f_k(t)\| \le M\; \forall t \in [0, 1],$$
and suppose that that the sequence \(\mu_k\) converges weakly to a measure  \(\mu\), then there exists a function \(f \in \LintRn\) such that \(d \mu = f dt\).
\label{thm:bounded_func_weakly_converge}
\end{thm}
\begin{proof}
  Let $\{f_k\}$ be a sequence of functions satisfying the condition of the theorem.
  Consider the linear operator $I: C \rightarrow \mathbb R$ defined by
  $$I(g) \coloneqq \mu(g).$$

  By the Cauchy-Schwarz inequality, we have that
  $$|I(g)| \le \lim \int_0^1 |\langle f_n(t), g(t) \rangle| \; \rm{d}t \le M \int_0^1 \|g(t)\|^2 \; \rm{dt}.$$
  This proves that the operator $C$ is bounded, so that its domain can be extended to the set
  $$L_2 \coloneqq \{ g: \mathbb R^n \rightarrow \mathbb R \; | \; \int_0^1 \|g(t)\|^2 \rm{d} t < \infty \}.$$
  
  By the Riesz representation theorem, there exists a function $f \in L_2$ such that
  $$I(g) = \int_0^1 \langle f(t), g(t) \rangle \; \rm{d}t, \text{ i.e. } \rm{d}\mu = f \rm{d}t.$$
\end{proof}
% \begin{proof}
% First notice that by considering the sequence of functions \(\{\frac{M+f_k}{2M}\}\), we can assume without loss of generality that \(0 \le \|f_k(t)\| \le 1\) for all \(n \in \mathbb N\). Furthermore, by considering the each entry independently, we can consider that the dimension $n$ is equal to 1.

% Denote the Lebesgue measure on \([0, 1]\) by \(\lambda\). The Radon-Nikodym Theorem states that \(\mu\) admits a density \(f(t)\) with respect to \(\lambda\) if and only if \(\lambda(A)=0\) implies \(\mu(A)=0\) for each subset \(A\) of \([0, 1]\). 

% We first show the result when \(A\) is open. For that, fix a subset \(A\) that satisfies \(\lambda(A) = 0\), and let's prove that \(\mu(A) = 0\).

% Notice that since \(0 \leq f_k \leq 1\) for all \(n \in \mathbb N\), then
% $$\mu_k(A) = \int 1_A(t) \cdot f_k(t) \, dt \leq \lambda(A) = 0.$$

% Portmanteau Theorem states that
% $$\mu(A) \leq \liminf_{n \to \infty} \mu_k(A).$$

% Which proves that \(\mu(A) = 0\). Now fix a subset \(B\) of \([0, 1]\) that need not to be open.

% Recall that \(\mu\) and \(\lambda\) are \emph{outer regular}, i.e.

% $$\mu(B) = \inf_{A \supseteq B, A \, \text{open}}\mu(A)  \text{ and } \lambda(B) = \inf_{A \supseteq B, A \, \text{open}}\lambda(A).$$

% For any open subset \(A\) of \([0, 1]\) such that \(A \supseteq B\),

% $$\mu(B) \leq \mu(A) \leq M \cdot \lambda(A).$$

% After taking the infimum on both sides with respect to \(A\), we get that \(\mu(B)=0\) for any set \(B\) satisfying \(\lambda(B)=0\).
% \end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "TV_SDP_v1"
%%% End:
\begin{lemma}
  Let $\{p_d\}$ be a sequence of univariate polynomials. If there exists a positive $\gamma$ such that for every $d \in \mathbb N$ the following holds
  $$\int_0^1 p_d q \le \int_0^1 q \quad \text{ for every $p$ of degree less than $d$},$$
  then the sequence $\{p_d\}$ has subsequence that weakly converges to a bounded function $h$.
\end{lemma}
\begin{proof}
  The ideas of the proof are inspired from \cite{noauthor_probability_nodate}.
To prove the claim it is sufficient to prove that the $i\text{-th}$ component of the $\{x^d\}$, i.e. the sequence of univariate functions $\{x^d_i\}$ , has a weak convergent subsequence. without loss of generality, assume that $i=1$.
  
For simplicity, define
$$\mu_d(g) \coloneqq \int_0^1 g p_d dt$$
for all $d \in \mathbb N$ and $g \in \LintRn$. If $g$ is a polynomial of degree no more than $d$, let $m$ be the maximum value of $\|g\|_{\infty}$ on the interval $[0, 1]$ so that $m - g$ is nonnegative, then $|\mu_d(g)| = |\mu_d(m)| + |\mu_d(m - g)| \le \gamma (m + \int_0^1 (m-g)) \le 2 m \gamma$.

Let $f_0, f_1, \ldots$ be a countable sequence of polynomial that is dense in $\LintRn$. Without loss of generality, we assume that the degree of $f_i$ is no more than $i$.
Consider the sequence of real numbers  $\{\mu_i(f_0)\}_{i \ge 0}$. This sequence is bounded by $2\gamma \max_{t \in [0, 1]} \|f_0(t)\|_\infty$. As such, it has a convergent subsequence $\mu_i^{(1)}$.

Next, we consider $\{\mu_i^{(1)}(f_1)\}_{i \ge 1}$. Again, this is a bounded sequence of real numbers and so it has a convergent subsequence $\{\mu_i^{(2)}(f_1)\}_{i \ge 1}$.

In this way, we obtain for each $r \ge 0$ a  nested subsequences $\{\mu^{(r+1)}_i\} \subseteq \{\mu^{(r)}_i\}$ such that for every $j \le r$, $\mu_i^{(r)}(f_j)$ converges as $i \rightarrow \infty$. Now consider the diagonal sequence $\mu_i^{(i)}$. It is clear that $\mu_i^{(i)}(f_j)$ converges for every $j$.

Now we use the fact that $\{f_i\}$ is dense to show that actually $\mu_i^{(i)}(g)$ converges for all polynomial functions $g \in \LintRn$. Indeed, pick a $\varepsilon > 0$ and $f_j$ such that
$$\|f_j(t) - g(t)\|_\infty \le \varepsilon \quad \forall t \in [0, 1].$$

Since $\mu_i^{(i)}(f_j)$ converges, there exists $N > 0$ such that if $i, i' \ge M$ then
$$|\mu_i^{(i)}(f_j) - \mu_{i'}^{(i')}(f_j)| \le \varepsilon.$$

Thus we have 
$$|\mu_i^{(i)}(g) - \mu_{i'}^{(i')}(g)| \le |\mu_i^{(i)}(g) - \mu_{i}^{(i)}(f_j)| + | \mu_{i}^{(i)}(f_j) -  \mu_{i'}^{(i')}(f_j)| + | \mu_{i'}^{(i')}(f_j) - \mu_{i'}^{(i')}(g)|$$


Without loss of generality, assume that $N$ is larger than the degree of $g$ as well, so that
$\mu_i^{(i)}(g - f_j) \le 2 \gamma \varepsilon$.

We conclude that 
$$|\mu_i^{(i)}(g) - \mu_{i'}^{(i')}(g)| \le 6\gamma \varepsilon,$$
so $\mu_i^{(i)}(g)$ converges.

To complete the proof, write $\mu^{\infty}(g) = \lim_i \mu_i^{(i)}(g)$ for every polynomial $g \in \LintRn$.
By construction, $\mu^{\infty}$ satisfies
$$|\mu^{\infty}(g)| \le \int_0^1 g,$$
for every polynomial $g$ that is nonnegative on $[0, 1]$.
Theorem 3.12 b) in LASSERRE proves that there exists a bounded function $h$ such that $\mu^{\infty}(g) = \int_0^1 gh$.
\end{proof}
We now go back to the proof of the Theorem.



---------------------
Indeed, pick a $\varepsilon > 0$ and $f_j$ such that
$$\|f_j(t) - g(t)\|_\infty \le \varepsilon \quad \forall t \in [0, 1].$$

Since $\mu^{i, (i)}(f_j)$ converges, there exists $N > 0$ such that if $i, i' \ge N$ then
$$|\mu^{i, (i)}(f_j) - \mu^{i', (i')}(f_j)| \le \varepsilon.$$
Without loss of generality, assume that $N$ is larger than the degree of $g$ as well, so that
$\mu^{i, (i)}(g - f_j) \le \varepsilon$. thus we have 
\begin{align*}
  |\mu^{i, (i)}(g) - \mu^{i', (i')}(g)| &\le |\mu^{i, (i)}(g) - \mu_{i}^{(i)}(f_j)| + | \mu_{i}^{(i)}(f_j) -  \mu^{i', (i')}(f_j)| + | \mu^{i', (i')}(f_j) - \mu^{i', (i')}(g)|
  \\& \le 3\varepsilon,
\end{align*}
so $\mu^{i, (i)}(g)$ converges.

